Structured Prompt Tuning

We propose structured prompt tuning, a simple and effective method to improve prompt tuning. Instead of prepending a sequence of tunable embeddings to the input, we generate the soft prompt embeddings through a hypernetwork. Our approach subsumes the standard prompt tuning, allows more flexibility in model design and can be applied to both single-task and multi-task training settings. Empirically, structured prompt tuning shows a gain of +1.2$~1.5 points on the GLUE benchmark and is less sensitive to the change of learning rate, compared to standard prompt tuning.

==> Makefile <==
.PHONY: all clean

DIST_DIR=dist

all: acl

watch:
	mkdir -p $(DIST_DIR)
	latexmk -quiet -bibtex -pvc -f -pdf \
		-pdflatex="pdflatex -synctex=1 -interaction=nonstopmode" \
		-output-directory=$(DIST_DIR) acl

acl:
	mkdir -p $(DIST_DIR)
	latexmk -quiet -bibtex -f -pdf \
		-pdflatex="pdflatex -synctex=1 -interaction=nonstopmode" \
		-output-directory=$(DIST_DIR) acl

clean:
	rm -rf $(DIST_DIR)

